GradPIM: A Practical Processing-in-DRAM Architecture for Gradient Descent

In this paper, we present GradPIM, a processing-in-memory architecture which accelerates parameter updates of deep neural networks training. As one of processing-in-memory techniques that could be realized in the near future, we propose an incremental, simple architectural design that does not invade the existing memory protocol. Extending DDR4 SDRAM to utilize bank-group parallelism makes our operation designs in processing-in-memory (PIM) module efficient in terms of hardware cost and performance. Our experimental results show that the proposed architecture can improve the performance of DNN training and greatly reduce memory bandwidth requirement while posing only a minimal amount of overhead to the protocol and DRAM area.

==> bufcmp/Evaluation.tex <==



\section{Evaluation}
\label{Evaluation}
%TABLE 1 at the Apps.tex
\vspace{-0.1em}
\input{Apps}

\subsection{Simulation Methodology}
We evaluated the performance and energy impact of buffered compares on a many-core CMP with simulation parameters displayed in Table~\ref{table:parameters}.
The system had 16 out-of-order cores, each running at 3GHz, with issue and commit width of 4 instructions per cycle. 
Each core had 16KB L1 I/D private caches, and 32MB L2 cache was shared in S-NUCA (2MB per core). 
The sizes of cache lines for both L1 and L2 caches were 64B.
We used McSimA+~\cite{mcsima+} for performance simulation, which we modified to support buffered compares.
McPAT~\cite{mcpat} was used for modeling the energy consumption of the cores, caches, and memory controllers at a 22nm logic process.
For DRAM timing and energy parameters, SPICE simulation was used. Refer to Table~\ref{table:spice} and Section~\ref{subsec:spice} for details.
%
We picked seven applications as explained in Section~\ref{sec:Apps}.


%\paragraph{Hashtable search -- contiguous key space:}
%\jinho{put a table about which app used which compare-n-action}
%\noindent\textbf{Hashtable search -- contiguous key space:}
%To represent hashtables with contiguous keys, we used a 4-way cuckoo hashtable similar to memc3~\cite{memc3}, a key-value store belonging to a memcached~\cite{memcached} family.
%To locate keys in a contiguous region, each set of four buckets has preallocated memory chunks to store keys.
%The Twitter dataset in Cloudsuite~\cite{cloudsuite} was used. % for set of search key distribution with twitter dataset.
%The simulation ran until all threads have finished 2,000 searches. 
%
%\noindent\textbf{Hashtable search -- non-contiguous keys:}
%Cuckoo hash-table in memc3 allocates a new memory region when a new item is added, which scatters the location of the keys. 
%Searching for non-contiguous keys with buffered compares was evaluated using the original hashtable from memc3, with all other parameters same to searching contiguous key space.   
%
%\noindent\textbf{B+ tree traversal:}
%B+ tree workload from Rodinia~\cite{rodinia} benchmark suite was selected for B+ tree traversal. 
%Simulation was run until 8,192 queries were finished by the threads.  
%
%
%
%\noindent\textbf{Find-or-put:}
%To examine find-or-put operation of buffered compares, ccTSA~\cite{ccTSA}, a DNA sequence assembler was used. 
%K-mer size was set to 27, and simulation was run until each thread consumed 100KB of data.
%
%\noindent\textbf{Large data:}
%Comparing a large data or copying data with buffered compares have a similar mechanism, and we examined this by increasing key sizes of the hashtable up to 256B, which spans up to four cache lines. 
 

 
\subsection{Overhead Analysis of Buffered Compares}
\label{subsec:spice}
To evaluate the energy overhead and timing parameters of BCUs, we conducted SPICE simulation on internal DRAM components. 
The inter-die I/O power values of the off-chip channels 
were from the latest DDR4 specifications~\cite{DDR4_spec}.
28nm DRAM process with 3 metal layers was used, 
and each 8Gb $\times8$ device had 16 banks and 8Kb pages with 6F DRAM cells. 
A modified version of the PTM low-power model~\cite{PTM} was used for the SPICE simulation. 
BCUs were modeled with key buffers, masks, arithmetic units, result queues, and command generators.  
The resulting energy and timing values are depicted in Table~\ref{table:spice}. 
Typical DRAM read energy $E_{rd}$ was divided into $E_{int\_bank}$ and $E_{int\_bus}$ 
where $E_{int\_bank}$ and $E_{int\_bus}$ represent internal access energy within a bank and internal access energy consumed on the bus connecting banks, respectively. 
We break down the energy into two parts because unlike ordinary DRAMs, buffered compare commands often access only an internal bank.
Energy consumption of a BCU per access is 0.3pJ, which is almost negligible compared to a data read energy of DRAM, which is 4nJ.
To read the key data and perform necessary calculations, BCUs incur a latency of 1.34 \nano\second~(tBCU) which is added to tCL to increase it by about 10\%. 
%However, this latency is added only when buffered compare operations are used, and does not increase latency of normal reads or writes. 
Note that the change in tCL does not affect the operating frequency of the DRAM.
%
The total area of all BCUs were 0.46 \milli\squaren\meter, which is only 0.53\% overhead of an 8Gb device,
where the total area of the DRAM was 86 \milli\squaren\meter ~with 50\% cell efficiency~\cite{DRAM_hynix}. 
The area of key buffers and comparators in BCUs were modeled using 22T TCAM model~\cite{TCAM_model}.
BC-light puts only one BCU at the chip I/O and increases the device area by 0.03\%, incurring negligible overhead. 
However, each BCU operation requires internal bus access, thus BC-light consumes a little more energy per operation than buffered compares.

\begin{table}%[tb!]
\small
\centering
\caption{DRAM parameters obtained from SPICE simulation}
\begin{tabular}{lclc}
\toprule
\multicolumn{2}{c}{Spec.} & \multicolumn{2}{c}{DDR4-2000} \\
\multicolumn{2}{c}{Process} & \multicolumn{2}{c}{28nm}\\
\midrule
%\multicolumn{2}{c}{Timing} & \multicolumn{2}{c}{Energy} \\
   Timing	& Value & Energy 			 & Value \\
\midrule
 tRCD				     & 14ns  & $E_{\text{ACT}}$                  & 12.5nJ     \\
 tRAS				     & 34ns  & $E_{\text{RES}}$                  & 30.0nJ     \\
 tRP				     & 14ns  & $E_{\text{PRE}}$                  & 7.5nJ      \\ 
 tCL				     & 14ns  & $E_{\text{compare}}$              & 0.3pJ      \\ 
 tBCU				     & 1.34ns & $E_{\text{int\_bank}}$            & 2.3nJ      \\ 
 tBL                                & 4ns   & $E_{\text{int\_bus}}$             & 1.9nJ      \\
 tRR                                & 1ns   & $E_{\text{IO}}$                   & 4.0nJ      \\
\bottomrule
\end{tabular}
\label{table:spice}
\end{table} 


To account for area/power overhead of memory controller for buffered compare, we conservatively used PARDIS~\cite{pardis}, a programmable memory controller comprised of two RISC processors, one for each of the frontend and transaction handling stages. 
For the PHY and the baseline memory controller, we used the models from McPAT~\cite{mcpat}. 
The area and power of the memory controllers are shown in Table~\ref{table:spice}. 


\subsection {Experimental Results}
%\figurename~\ref{fig:speedup}, \ref{fig:ext_bw}, \ref{fig:int_bw}, and \ref{fig:energy} show the experimental results. 
We compare our approach with the baseline where all computations are performed in the host processor without any NDP technique. We also compare our approach with two other NDP techniques that are implemented on a CPU die. 
First, we use active memory operations (\emph{AMO}) which allow memory controllers to perform memory-intensive computations \cite{AMO}.
For this, we put modules similar to BCUs at the memory controllers. 
We also compare our technique with active memory processor (\emph{AMP})~\cite{AMP}, where a specialized processor with its own 16MB cache is located in front of memory controller to handle buffered compare operations.  
We put enough resources into AMO and AMP to ensure that their computational capacities do not become the system bottleneck.
While a fine-grained accelerator can be another option, we decided not to add it because the benchmark applications were all memory-intensive and not likely to benefit from computational accelerators.

The baseline, active memory operations, active memory operation, active memory processor, buffered compare, and BC-light are marked as ``Baseline'', ``AMO'', ``AMP'', ``BC'', and ``BC-light''.


\begin{figure}
	\centering
	\includegraphics[width=.95\columnwidth]{figures/speedup} 
	\vspace{-2mm}
	\caption{Speedups of buffered compares. Values are normalized to performance of the baseline.}
	\vspace{-3mm}
	\label{fig:speedup}
\end{figure}



\subsubsection{Performance Analysis}
\begin{sloppypar}
\figurename~\ref{fig:speedup} shows speedups of buffered compares over the performance of the baseline system.
To show the effect of buffered compare on tCL increase, we also add the results of buffered compare where the tCL increase due to tBCU is neglected (BC-no\_tBCU). 

Buffered compares achieve significant speedup over the baseline and active memory operations. 
For three in-memory DB scan and aggregation workloads (TSC, TSR, and MAX), the speedups are especially high. 
In TSC, the speedup of BC is $6.87\times$. 
BC transfers to the host only the comparison results, instead of the whole data, thereby greatly reducing the amount of bandwidth used. 
In TSR, the benefit of BC is $6.62\times$, which is slightly lower than TSC.
%Buffered compare scheme functions similarly, but some unnecessary columns have to be fetched to the bank I/O even though it is not used by the BCU. 
Because the table is stored row-wise, large space exists between the two items of the same column. 
Thus much of the internal bandwidth is wasted and the speedup is decreased.
On the other hand, the baseline system cannot utilize the spatial locality of cache subsystem which was available in column-store, and this partially offsets the wasted internal bandwidth in BC.
The MAX workload shows the highest speedup for BC, which is 15.5 times the baseline.
When using compare-n-read, the range of data which can be processed by a single operation is usually bounded by the size of result queues.
Compare-n-select operation used for the MAX workload, on the other hand, does not return all the comparison results, but just the maximum value to the host. 
As a result, the range of data is only bounded by the size of DRAM page, which is the reason for such an outstanding speedup over other workloads. 
\end{sloppypar}


In BT, the speedup of BC is 35.9\%. In a B+tree node, hundreds of keys are placed sequentially in the DRAM, and therefore looking for the child node to descend can be very efficiently processed using compare-n-read.
Even though the baseline system uses binary search, the data stored in the node have to be fetched in the unit of cache lines, and the amount of data fetched to the host is much larger than BC, where only the comparison results are read. 

The speedup of BC on KV and SA workload are 20.5\% and $2.03\times$, respectively. 
Both workloads use hashtables as their data structure. 
Because searching hashtables finishes typically within a few reads, gains obtained by processing a wide range of data with buffered compare is not superior.
However, compare-n-increment gives additional benefits to BC, because performing the same operation with the baseline system would require both read and write to the memory, whereas BC only requires writing for filling the key buffer.

BC shows $4.11\times$ speedup on HT. 
Using BC, the data have to be accessed multiple times to count the number of items for each histogram bin. 
Therefore, the amount of data accessed is actually larger in BC than the baseline. 
However, similar to the case in BT, the benefit of using less external bandwidth more than compensates for this loss and results in a superior performance.


The performance difference between BC and BC-no\_tBCU shows the amount of performance degradation cause by the tCL increase due to BCUs.
Overall, the change in tCL does not cause much slowdown since the system bottleneck is usually at the off-chip channel bandwidth.
The latencies added are usually hidden by transfers from other banks. 
In geometric mean, tBCU accounts for 1.8\% loss in speedup. 



\begin{sloppypar}
BC-light shows speedup for five workloads, TSC, MAX, KV, SA, and HT, which are $1.80\times$, $2.25\times$, 15.5\%, $2.01\times$, and 26.6\%, respectively. 
BC-light only utilizes rank-internal bandwidth instead of the bank-internal bandwidth, and the obtained speedup is less than BC.
In TSR, the unnecessary data fetch to the chip I/O occupies the internal bus of the DRAM devices, and the rank internal bandwidth becomes the bottleneck yielding negative gain.
Actually, if more than four ranks are used per memory channel, the gain can be positive.
When eight ranks were used instead of four ranks per channel, it gets 42.4\% performance speedup.
Similarly in BT, the required internal bandwidth of sequential search is much larger than the binary search. In BC, the abundant number of banks can provide sufficient internal bandwidth, but in BC-light, the amount of internal bandwidth is simply not enough.
\end{sloppypar}


AMO does not show much speedup over the baseline, and it shows negative gains for most workloads. 
By processing at the memory controller on the host side, active memory operations does not reduce the number of memory accesses.
Furthermore, it cannot benefit from temporal locality of the on-chip caches. 
Therefore, the active memory operation does not provide speedup for the evaluated workloads. 

The trend is not different for AMP in that it does not dramatically reduce the number of memory accesses. 
However, having its own cache reduces some memory accesses and mitigates the drawback of AMO. 
As a result, AMP gains performance by about 16\% on geometric mean by reducing the on-chip network delays between cores and the memory controller.

\begin{figure}
	\centering
	\includegraphics[width=.95\columnwidth]{figures/ipc} 
	\vspace{-2mm}
	\caption{Aggregate IPC values.}
	\vspace{-3mm}
	\label{fig:ipc}
\end{figure}


\figurename~\ref{fig:ipc} shows the aggregate IPCs over all cores (16 cores). 
BC shows the highest IPC, because of its superior performance in memory-intensive operations over others.
On the other hand, the baseline shows relatively high IPC despite its low performance. 
This means that there is no offloading and all the computation is done at the processor cores.
%Note that the IPC values are not high enough to cause contention at the computing resources.


\begin{figure}
	\centering
	\includegraphics[width=.95\columnwidth]{figures/ext_bw}
	\vspace {-3mm}
	\caption{External bandwidth usage.}
	\vspace {-3mm}
	\label{fig:ext_bw}
\end{figure}



\begin{figure}
	\centering
	\includegraphics[width=.95\columnwidth]{figures/int_bw}
	\vspace {-3mm}
	\caption{Internal bandwidth usage. Internal bandwidth is measured by aggregating the amount of data fetched from cells to bank I/O.}
	\label{fig:int_bw}
	\vspace {-4mm}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=0.99\columnwidth]{figures/mcutil}
	\vspace{-5mm}
	\caption{DRAM command rates. The values are normalized to the maximum rate (sending a command every cycle) of a baseline memory controller. Command rates of BC and BC-light are divided into commands from the memory controller (ext.) and from the all command generators (int.). }
	\vspace{-3mm}
	\label{fig:mcutil}
\end{figure}



\begin{figure}
	\centering
	\includegraphics[width=.95\columnwidth]{figures/mpki}
	\vspace {-3mm}
	\caption{Number of memory access operations. The light gray bar shows the number of memory access per kilo instructions (MAPKI) for the baseline and the dark gray bar shows the number of buffered compare operations per kilo instructions (BPKI). }
	\label{fig:mpki}
	\vspace {-4mm}
\end{figure}




\subsubsection{External and Internal Memory Bandwidth}
%\figurename~\ref{fig:ext_bw} and \ref{fig:int_bw} show external and internal memory bandwidth usage, respectively. 
By internal bandwidth usage, we mean the amount of data read from the bank to the bank I/O or written backwards, either by buffered compare commands or normal read/writes.
\figurename~\ref{fig:ext_bw} shows that the external bandwidth is saturated for most workloads with the baseline, AMO, and BC. In contrast, BC-light shows very low external bandwidth utilization.
\figurename~\ref{fig:int_bw} shows an idea why high speedup can be achieved with BC. 
The internal bandwidth usages have a strong correlation with the speedup achieved over the baseline. The internal bandwidths used by BC are several times higher than the peak external bandwidth, which cannot be obtained without PIM.
\figurename~\ref{fig:mcutil} explains how BC exploits such high internal bandwidth, where BC exhibits very high aggregate internal command rates.  The command generator at each bank commands the column select and arithmetic operations needed for exploiting the internal bandwidth.  
\figurename~\ref{fig:mpki} shows another insight by comparing the number of memory accesses per kilo instructions (MAPKI) of the baseline and the number of buffered compare operations per kilo instructions (BPKI). 
Even though the number of instructions for baseline and BC are not exactly the same as BC uses special instructions, having less memory accesses allow BC to make faster progress. 

On the other hand, the baseline, AMO and AMP consume exactly the same amount of internal bandwidth and external bandwidth. This is because any data to be used need to traverse all the way from cells to the memory controller, or in the opposite direction. In BC-light, the internal bandwidth usage is larger than the peak external bandwidth, which is the reason for its speedup in some workloads. However, its peak internal bandwidth is only a few times the maximum external bandwidth, while the internal bandwidth of BC is tens of times the external bandwidth. The rank-internal bandwidth becomes the bottleneck, and thus BC-light cannot fully utilize the external bandwidth.

\figurename~\ref{fig:memlat} describes where the time is spent inside DRAM for the buffered compare operations.
The queuing delays for key buffer write and result retrieval consume the longest latency.
It is because they compete for external bandwidth which is the system bottleneck.  
Result retrieval waits shorter than key buffer writes, because result retrievals are prioritized over key buffer writes so that the bank and the BCU can serve other requests.
Even though fetching the data and performing comparison is done over a long range of data, they only require bank-local resources and thus the latency is usually not significantly long.

\begin{figure}
	\centering
	\includegraphics[width=.75\columnwidth]{figures/memlat} 
	\vspace{-2mm}
	\caption{Breakdown of buffered compare execution time inside DRAM.}
	\vspace{-3mm}
	\label{fig:memlat}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=.99\columnwidth]{figures/energy}
	\vspace{-6mm}
	\caption{Normalized energy consumption breakdown. Values are normalized against baseline.}
	\label{fig:energy}
	\vspace{-6mm}
\end{figure}



\subsubsection{Energy Consumption}
\figurename~\ref{fig:energy} shows the breakdown of energy consumption normalized to the baseline. 
The major source of power consumption is the cores, which depends on IPC and the execution time. 

BC achieves a large reduction in energy consumption, up to 94.7\% in MAX, and 74.7\% in geometric mean.
The reason for such reduction is twofold: saving in static energy due to the reduced run time and dynamic energy reduction from computation offloaded to the memory.
There is no significant difference in energy consumed in the memory, but BC decreases it by a small amount, since the number of off-chip accesses is reduced.
The only exception is BT, where BC consumes a little bit more energy in the memory than the baseline. 
The energy reduction in off-chip accesses is offset by the increased number of internal reads, 
because BC performs a sequential search while the baseline uses binary search.
BC-light shows similar trends with BC, but in TSR and BT workloads, its negative performance gain also results in an energy increase. In geometric mean, 39.8\% of energy reduction is obtained on BC-light.
%Buffered compares tend to access more data from the cells, but it is offset by fewer PMI accesses.
AMO and AMP, however, do not show clear advantages over the baseline. 
While the reduction of the energy consumption is observed in some applications, most of it is coming from the offloading of computations and reduction in execution times. 
Although the energy consumptions of the memory controllers are shown, they are amortized over other parts of the processor. 
The portion of the memory controller in energy consumption was less than 0.2\% throughout the benchmarks.


\begin{figure}
	\centering
	\includegraphics[width=0.99\columnwidth]{figures/sense2}
	\vspace{-5mm}
	\caption{Speedup depending on number of banks, ranks, and channels. Values are normalized to 1MC 4r-16b for each application.}
	\label{fig:sense-rb}
	\vspace{-2mm}
\end{figure}





\subsubsection{Sensitivity to the Number of Banks, Ranks, and Channels}

Buffered compare scheme utilizes bank-internal bandwidth to read the data to be processed, and use external bandwidth to fill key buffers and read the results.
Consequently, the performance of buffered compare operations is sensitive to both the internal and external bandwidth, and the sensitivity depends on the application characteristics.
%\figurename~\ref{fig:sense-rb} shows the speedup of two representative appslications, TSR and KV with the geometric mean of the six all applications using different number of ranks, banks, and memory channels.
\figurename~\ref{fig:sense-rb} shows the performance of the BC using different number of ranks, banks, and memory channels, normalized to one memory channel, four ranks and 16 banks per rank.
%BCUs are placed at the edge of each bank, and multi-bank architecture is the key for providing the fertile internal bandwidth.
As the number of ranks and the number of banks per rank change, the amount of internal bandwidth also scales and the increased number of memory channels results in more external bandwidth.
KV does not demand so much internal bandwidth as displayed in \figurename~\ref{fig:int_bw}, and thus less sensitive to the internal bandwidth and more sensitive to the external bandwidth.
When the number of ranks is increased, its performance slightly drops in some configurations because of rank-to-rank switching delay.
On the other hand, curves for TSR shows that it is very sensitive to the provided internal bandwidth. 
When the number of banks and ranks increases, the speedup sharply rises. 
Even when more channels are provided, the performance degrades if aggregate number of banks is smaller (compare 1MC 4r-16b and 2MC 1r-8b).
On average, the performance depends more on the number of channels, because the external bandwidth is usually the bottleneck.




%\subsubsection{Sensitivity to Number of Memory Channels}
%As number of channels increase, performance goes up.




%\begin{figure}
%	\centering
%	\includegraphics[width=0.39\columnwidth]{figures/BWperreq}
%	\caption{The amount of bandwidth required per processing a request.}
%	\label{fig:BWperreq}
%\end{figure}


\subsubsection{Sensitivity to Data Size}

%\jinho{is this section needed?}



\begin{figure}
	\centering
	\includegraphics[width=0.60\columnwidth]{figures/rate}
	\vspace{-2mm}
	\caption{Speedups according to the data size.}
	\label{fig:rate}
	\vspace{-4mm}
\end{figure}



Each buffered compare operation requires off-chip accesses to fill the key buffer and retrieve the results, which becomes the performance bottleneck. 
Thus, it is beneficial to process as many data as possible in one operation.
\figurename~\ref{fig:rate} shows the speedup over the baseline of TSC, TSR, and MAX, according to the size of data. 
For TSC and MAX, the data size represents the column only, and for TSR, the data size is the whole table.
In TSC, compare-n-read is used for small items, and in this case, the result queue becomes the limiting factor.
If the number of items exceeds the size of a result queue, the buffered compare operation is split, and thus further increasing the data size does not increase the speedup.



On the contrary, in a row-store table, only a few items are stored inside a DRAM page, and thus the data processed per compare-n-read operation is bounded by the DRAM page size in TSR.
MAX workload uses compare-n-select, which does not utilize the result queue. 
Because of this, the data size limiter is again the DRAM page.






%
%       \begin{table}%[tb!]
%       \small
%       \centering
%       \caption{DRAM parameters obtained from SPICE simulation}
%       \begin{tabular}{llc}
%       \toprule
%       \multicolumn{2}{l}{Timing} & Energy \\
%       \multicolumn{4}{l}{Parameter} & Value & Parameter & Value \\
%       \midrule
%       \multicolumn{3}{l}{DRAM:} \\
%        & process 			     & 29nm  \\
%        & tRCD				     & 14ns  \\
%        & tRAS				     & 34ns  \\
%        & tRP				     & 14ns  \\
%        & tCL				     & 14ns  \\
%        & tBCU				     & 1.34ns \\
%        & $E_{\text{ACT}}$                  & 12.5nJ     \\
%        & $E_{\text{RES}}$                  & 30.0nJ     \\
%        & $E_{\text{PRE}}$                  & 7.5nJ     \\
%        & $E_{\text{compare}}$              & 0.7pJ     \\
%        & $E_{\text{int\_bank}}$       & 2.3nJ     \\
%        & $E_{\text{int\_bus}}$        & 1.9nJ     \\
%        & $E_{\text{IO}}$                   & 4.0nJ     \\
%       \bottomrule
%       \end{tabular}
%       \label{table:parameters}
%       \end{table} 
%
%
%
%


==> index.tex <==


\begin{figure*}

\large

     \fbox{\begin{minipage}{0.95\textwidth}We sincerely thank the reviewers for their time and valued comments. We have faithfully revised our paper and addressed each reviewers' comments below with much appreciation. All the revised texts are written in {\color{olivegreen}green color} with magenta markers {\color{magenta}{R1-R10}} around them. Please find the index below with \underline{hyperlinks} to them. \end{minipage}} 

\vspace{5mm}

\underline{\huge\textbf{\textsf{Index}}}
\vspace{3mm}
\begin{enumerate}
\item \textbf {Results for full precision training (reviewer D,E):} 
\begin{itemize}
\item \revref{R1a} (p.2, right), 
\item \revref{R1b} (p.10, left), 
\item \revref{R1c} (p.10, right),
\item \figref{analysis}
\item \figref{sense:precE} 
\end{itemize}

\item \textbf {Split the benefit of BGLP and architecture design (reviewer C):} 
\begin{itemize}
\item \revref{R2a} (p.7, right)
\item \revref{R2b} (p.8, right) 
\item \revref{R2c} (p.9, left)
\item \figref{perf}
\end{itemize}

\item \textbf {Analysis on per-bank vs per-bank group (reviewer D):}
\begin{itemize}
\item \revref{R2a} (p.7, right)
\item \revref{R3} (p.9, left)
\item \figref{perf}
\end{itemize}

\item \textbf {Energy for GradPIM-buffered (reviewer B,D):}
\begin{itemize}
\item \revref{R4a} (p.9, left)
\item \revref{R4b} (p.9, right)
\item \figref{energy}
\end{itemize}

\item \textbf {SIMD unit utilization (Reviewer B):}
\begin{itemize}
\item \revref{R5a} (p.9, right) 
\item \revref{R5b} (p.10, left)
\item \figref{subperf}-right
\end{itemize}

\item \textbf {Expandability of GradPIM for commercial success (reviewer A,D):}
\begin{itemize}
\item \revref{R6a} (p.1, left)
\item \revref{R6b} (p.11, right)
\end{itemize}


\item \textbf {Other parameter update algorithms (reviewer C): }
\begin{itemize}
\item \revref{R7} (p.11, right)
\end{itemize}


\item \textbf {Buffer for GradPIM (reviewer B): }
\begin{itemize}
\item \revref{R8} (p.8, left)
\end{itemize}


\item \textbf {8bit quantization affecting the accuracy (reviewer E):}
\begin{itemize}
\item \revref{R9} (p.2, right)
\end{itemize}

\item \textbf {Comparison with other accelerators (reviewer D,E):}
\begin{itemize}
\item \revref{R10} (p.10, left)
\item \figref{sense:ratio}
\end{itemize}

\item \textbf {Baseline used for normalization \figurename~\ref{fig:sense:ratio} (reviewer E): }
\begin{itemize}
\item \revref{R10} (p.10, left) 
\item \figref{sense:ratio}
\end{itemize}
\end{enumerate}
\end{figure*}

==> sections/oldProcedure.tex <==
\circled{1} Two rows are activated, effectively loading the weights $\theta_t$ and $v_t$ into the row buffers. 
%Since they are placed in difference banks, both the rows can remain open at the same time. 
\circled{2} The gradients $g$ are written to the registers scaled by $\eta$, using scaled\_wr command. Even though each gradient is 8 bits, they are stored in 32bit width to the register so that it can be computed in parallel with the other elements.
\circled{3} A column of $\theta_t$ is loaded to one of the registers, scaled by ($-\eta\beta$) \JL{load negative? or vector subtract?} using scaled\_rd operation. 
\circled{4} The scaled values in the two registers above are processed with vector\_add, creating the second term for the Eq.~\ref{eq:?}.
\circled{5} A column of $v_t$ is loaded into a register, scaled by $\alpha$. 
Then it is vector\_added to the register of step 4 to create $v_{t+1}$.
\circled{6} Write\_back performed to the register with $v_{t+1}$ on the open row for the $v_t$.
\circled{7} Similarly, a column of $\theta_{t+1}$ is generated by Equation~\ref{eq:?} and written back in the place of $\theta_t$.
Finally, \circled{2} - \circled{7} is repeated for consecutive columns of $\theta$ and $v$ until the entire row has been processed. 

==> sections/trash.tex <==


\subsection{mixed-precision Training}
mixed-precision training is becoming increasingly popular in DNN training aimed at low-energy training.
However, as the precision of the data used in DNN training decreases, it is known to suffer from accuracy drop due to quantization errors.
Lowering the precisions of activations, gradients and weights are all in general known to pose separate challenges. 
However, the common consensus is that the master weights need larger precision, while the gradients are the most forgiving to the quantization errors, as demonstrated in ~\cite{baidu} with 16-bit training with 32-bit master weights. 
\cite{ibm1} is one popular work which uses 8-bit floating point format for all executions, but keeps the master weight at 16 bits to mitigate the swamping effect~\cite{swamping}. % Nicholas J Higham. The accuracy of floating point summation. SIAM Journal on Scientific Computing, 14 (4):783–799, 1993.
In \cite{ibm1}, techniques called chunk-based accumulation and floating point stochastic rounding are introduced, where the former organizes the order of the additions to reduce the average gap of range between the two add operands, and the latter alleviates the loss coming from a smaller number being added to a larger number.
Later, \cite{intel1} suggested improved rules for loss scaling and stochastic rounding, and \cite{ibm2} proposes a custom floating point format that provides a better dynamic range for the training.
In addition, there is work on using a hybrid of floating point and fixed point precision~\cite{intel2} because low precision fixed point format has better precision than floating point format but lacks the dynamic range.

In this work, we adopt 8-bit floating point training while maintaining 32-bit fixed point master weight, which stably provides a good accuracy with relatively low hardware cost.
Also, we adopt widely used techniques such as chunk-based accumulation, and custom floating point formats for our training.



\JL{maybe remove this} Mixed-precision training~\cite{ibm1, ibm2, intel1, intel2, baidu} is a major research field regarding NPU technology.
Mixed-precision training performs numeric operations in low precision while keeping a copy of their master weights in high precision. 
It can preserve training accuracy while reducing computational costs and memory bandwidth consumption.
NVIDIA TensorCore~\cite{tensorcore} is a direct example of a mixed-precision training algorithm that is being applied to GPUs today. It performs 16-bit operations and 32-bit accumulation to obtain a performance boost. 
Such techniques are being extensively used in many cases~\cite{4min, 224sec}, contributing to the reduction in DNN training cost. There are also a few attempts aimed at further reducing training data precision to 8 bits~\cite{ibm1, ibm2}. 
By applying techniques such as custom floating-point representation and chunk-based accumulations, quantization error can be mitigated to achieve almost no accuracy loss with 8-bit datapaths.


    \begin{comment}
    The register store command is similar to the column write command, except that it writes to a temporary register instead of the cells. 
    Therefore the command is governed by tCWD, tBURST since it occupies the data bus. 
    
    Similar to the scaled read command, we assign tCCD\_S for the register store.
    However, it only occupies the global I/O gating. Thus a register store command can overlap with the scaled read command since they do not share any circuitry in common. 
    On the other hand, the register store commands to different bank groups cannot happen in an overlapping way, since they share the global I/O gating in the datapath.
   % Similar to waiting for tRTP, we assume the write to the register is complete after tWR time, which also leave a large timing margin since it does not need the sense amplifiers to function. However, any following precharge operation does not have to wait for the tWR time after the scaled wr, since the sense amplifiers and the bitlines have never been occupied.
    Also, register store command is not affected at all by tRAS since it has no interaction with the cells.
    \end{comment}

==> trash.tex <==
\begin{comment}
To alleviate the problem, numerous solutions have been proposed. 
Distributed training~\cite{distributed} is one of them, which exploits the vast amount of data-parallelism with multiple GPUs to obtain the speedup~\cite{ddl1, ddl2, ddl3}.
However, it requires high-end interconnection between the nodes to scale beyond a few GPUs.
In addition, using multiple GPUs in parallel is by no means energy-efficient~\cite{224sec}.


\end{comment}

\JL{GPU: 16bit, NPU: 8bit+ something special}
\JL{distrib exist for for GPU and NPU} 




Also, quantization~\cite{q1, q2, mix1, mix2, yoo} is another way to reduce both the computation and the memory burden of the DNNs, by reducing the precision of each parameter and activations. 
However, quantization often suffers from accuracy drop, and have to be selected carefully on how much quantization should be applied.
